Cyclotron Radiation Emission Spectroscopy of Electrons from Tritium Beta Decay and $^{83\rm m}$Kr Internal Conversion

Project 8 has developed a novel technique, Cyclotron Radiation Emission Spectroscopy (CRES), for direct neutrino mass measurements. A CRES-based experiment on the beta spectrum of tritium has been carried out in a small-volume apparatus. We provide a detailed account of the experiment, focusing on systematic effects and analysis techniques. In a Bayesian (frequentist) analysis, we measure the tritium endpoint as $18553^{+18}_{-19}$ ($18548^{+19}_{-19}$) eV and set upper limits of 155 (152) eV (90% C.L.) on the neutrino mass. No background events are observed beyond the endpoint in 82 days of running. We also demonstrate an energy resolution of $1.66\pm0.19$ eV in a resolution-optimized magnetic trap configuration by measuring $^{83\rm m}$Kr 17.8-keV internal-conversion electrons. These measurements establish CRES as a low-background, high-resolution technique with the potential to advance neutrino mass sensitivity.

==> packages.tex <==
\usepackage{color}
\usepackage{graphicx}% Include figure files
\usepackage{upgreek}
\usepackage{lineno} % FIXME: remove before arXiv post
\usepackage{pifont}
\usepackage{siunitx}
\usepackage{blindtext}
%\usepackage{multirow, booktabs, makecell, caption}

%Revtex4-2 is incompatible with this package, produces errors about \prevdepth.
